Vehicle Fault-Tolerant Robust Power Transmission Line Inspection Planning

This paper concerns fault-tolerant power transmission line inspection planning as a generalization of the multiple traveling salesmen problem. The addressed inspection planning problem is formulated as a single-depot multiple-vehicle scenario, where the inspection vehicles are constrained by the battery budget limiting their inspection time. The inspection vehicle is assumed to be an autonomous multi-copter with a wide range of possible flight speeds influencing battery consumption. The inspection plan is represented by multiple routes for vehicles providing full coverage over inspection target power lines. On an inspection vehicle mission interruption, which might happen at any time during the execution of the inspection plan, the inspection is re-planned using the remaining vehicles and their remaining battery budgets. Robustness is introduced by choosing a suitable cost function for the initial plan that maximizes the time window for successful re-planning. It enables the remaining vehicles to successfully finish all the inspection targets using their respective remaining battery budgets. A combinatorial metaheuristic algorithm with various cost functions is used for planning and fast re-planning during the inspection.

==> tbl/distance_table.tex <==
\begin{tabular}{l  r r r r r r r r r}
   \noalign{\hrule height 1.1pt}\noalign{\smallskip}
   \Dmax [\si{m}] & 500 & 600 & 700 & 800 & 900 & 1\,000 & 1\,200 & 2\,000 & 5\,000\\
   %\hline
   $n_{s}$ & 15 & 23 & 28 & 33 & 40 & 43 & 51 & 76 & 172\\
   \noalign{\hrule height 1.1pt}
\end{tabular}


==> tbl/result_data.tex <==
{500}&{15}&{100}&{4}&{20}&{58}&\textbf{66}\\ 
{700}&{28}&{200}&{4}&{17}&{86}&\textbf{100}\\ 

